Textless Speech Emotion Conversion using Discrete and Decomposed Representations

Speech emotion conversion is the task of modifying the perceived emotion of a speech utterance while preserving the lexical content and speaker identity. In this study, we cast the problem of emotion conversion as a spoken language translation task. We use a decomposition of the speech signal into discrete learned representations, consisting of phonetic-content units, prosodic features, speaker, and emotion. First, we modify the speech content by translating the phonetic-content units to a target emotion, and then predict the prosodic features based on these units. Finally, the speech waveform is generated by feeding the predicted representations into a neural vocoder. Such a paradigm allows us to go beyond spectral and parametric changes of the signal, and model non-verbal vocalizations, such as laughter insertion, yawning removal, etc. We demonstrate objectively and subjectively that the proposed method is vastly superior to current approaches and even beats text-based systems in terms of perceived emotion and audio quality. We rigorously evaluate all components of such a complex system and conclude with an extensive model analysis and ablation study to better emphasize the architectural choices, strengths and weaknesses of the proposed method. Samples are available under the following link: https://speechbot.github.io/emotion.

==> 01.intro.tex <==
\section{Introduction}
\label{sec:intro}
\begin{figure}[t!]
\centering
\resizebox{0.45\textwidth}{!}{%
  \includegraphics[width=\linewidth]{figs/arch.png} 
%   \includegraphics[width=\linewidth]{figs/model_zoom.png}  
}
\caption{An illustration of the proposed system. 

We use pink to denote models and green to denote representations.}
\vspace{-0.4cm}
\label{fig:arch}
\end{figure}

Speech signals carry information beyond the lexical content. Such information is often contained in various attributes: speaker identity, prosodic features, timbre, recording conditions, etc. Modifying the above attributes might completely alter the meaning of the speech utterance. For example, consider the sentence: ``Well, this is great''. Keeping the content fixed, the intent of the speaker is perceived differently when uttered in an angry or an amused acted emotion. This phenomenon was studied in the psychoacoustic literature, where \citet{mehrabian1967decoding} showed that the perceived emotion often overrides the speech content.

Generating natural speech is a fundamental building block in improving human-computer interaction~\cite{tits2019theory}. Modeling emotion in speech is arguably one of the main challenges in developing more natural and expressive speech synthesis models. Although speech based generative models have shown great success in recent years~\cite{skerry2018towards, fastspeech2, kim2021expressive, sorin2020principal, hono2020hierarchical}, the majority is still text-based, i.e., text-to-speech~\cite{tan2021survey}, and is therefore limited in terms of expressivity. This is due to being restricted to what can be expressed and annotated in text.

The task of speech emotion conversion involves with modifying the perceived emotion of a speech utterance while preserving the speaker identity and the lexical content~\cite{zhou2021emotional}. Current methods are mainly based on manipulating parameters of the speech signal~\cite{inanoglu2009data, aihara2012gmm, gao2018nonparallel, robinson2019sequence, rizos2020stargan, zhou2020transforming, zhou2020converting, zhou2021limited, zhou2021seen, zhou2021vaw}. Such modeling approach was shown to be effective for voice conversion~\cite{polyak2019tts, sisman2020overview} and singing voice conversion~\cite{polyak2020unsupervised}.
Although these methods presented impressive generation capabilities, such modeling does not explicitly account for non-verbal vocalizations (e.g., laughter, crying, yawning) as it is content-agnostic. Ideally, such a model should be able to insert, remove, or replace non-verbal cues representing different emotions.

In this work we focus on the task of speech emotion conversion and modeling under the parallel dataset setting. Following recent success in textless spoken language modeling~\cite{gslm, gslm2, gslm3}, we suggest: (i) a novel textless approach for decomposing speech into a disentangled and discrete representation, accounting for both content and prosody; (ii) modeling emotion conversion as a \emph{spoken language translation} task using Natural Language Processing methods; (iii) directly synthesizing expressive speech from discrete representations (no spectrogram estimation). The above modeling scheme allows us for the first time to directly modify emotion-related content units, while controlling  attributes such as speaker identity, F0, and timbre.

Results suggest that the proposed method is superior to the evaluated baselines. We conducted an extensive evaluation of the modules composing our system, and conclude with an ablation study to better understand the effect of each component of the decomposition on the overall generated speech. 

\noindent{\textbf{Our contributions:}}
We propose a novel textless approach by casting the task of speech emotion conversion as a \emph{spoken language translation} problem. We demonstrate how such a paradigm can be used to model expressive non-verbal communication cues as well as generating high-quality speech samples. Finally, we empirically demonstrate the efficacy of the proposed method using both objective and subjective measures.

==> 03.mode.alt.tex <==
\vspace{-0.1cm}
\section{Model}
\label{sec:model}
As emotion manifests itself in multiple aspects of spoken language, to optimally convert emotion one needs to consider all aspects in the conversion process. For example, emotion can be expressed via a prosodic features (high pitch, slow speaking rate, etc.), speaking style (yelling, whispering, etc.), and non-verbal vocalizations (laughing, yawning, crying, etc.).

We propose to decompose the speech signal into four components: phonetic-content, prosodic features (i.e., F0 and duration), speaker identity, and emotion-label, denoted by $\zc, (\zdur, \zf), \zspk, \zemo$ respectively. 
Using the above decomposition we propose the following cascaded pipeline: (i) translate non-verbal vocalizations in $\zc$ while preserving the lexical content (e.g., when converting from amused to sleepy, we remove laughter and insert yawning); (ii) predict the prosodic features of the target emotion based on the translated content; (iii) synthesize the speech from the translated content, predicted prosody, target speaker identity and target emotion-label.

% Consecutive occurrences of the same token are collapsed to a single token. Next, we feed this representation to a sequence-to-sequence Transformer model optimized for translating discrete representations of different emotions. We predict the durations of each token in the translated output sequence and inflate them accordingly. Using a F0 estimation model and the translated tokens, we predict the F0 corresponding to the target emotion. Finally, we feed them together with the target speaker-embedding and target emotion-token to a neural vocoder trained to reconstruct the time-domain audio signal. The overall architecture is depicted in Figure~\ref{fig:arch}.

\vspace{-0.1cm}
\subsection{Speech Representation}
\paragraph{Phonetic-content representation.}
To represent speech phonetic-content we extract a discrete representation of the audio signal using a pre-trained \ac{SSL} model, namely HuBERT. We use a \ac{SSL} representation for phonetic-content in order to capture non-verbal vocalizations (unlike text where they are often not annotated). We discretize this representation for better modeling and sampling (as opposed to regressing on continuous variables). This paradigm allows us to benefit from all recent advances in \ac{NLP}.

Denote the domain of audio samples by $\mathcal{X} \subset \mathbb{R}$. The representation for an audio waveform is therefore a sequence of samples $\x = (x^1, \dots, x^T)$, where each $x^i \in \mathcal{X}$ for all $1 \leq t \leq T$. The content encoder $E_c$ is a HuBERT model \cite{hsu2020hubert} pre-trained on the LibriSpeech corpus~\cite{Panayotov2015}. HuBERT is a self-supervised model trained on the task of masked prediction of continuous audio signals, similarly to BERT~\cite{bert}. During training, the targets are obtained via clustering of MFCCs features or learned representations from earlier iterations.
The input to the content encoder $E_c$ is an audio waveform $\x$, and the output is a spectral representation sampled at a lower frequency $\z' = (z_c^{'1}, \dots, z_c^{'L})$ where $L < T$. Since HuBERT outputs continuous representations, an additional k-means step is needed in order to quantize these representations into a discrete unit sequence denoted by $\zc = (z_c^1, \dots, z_c^L)$ where $z_c^i \in \{1, \dots, K\}$ and $K$ is the size of the vocabulary. For the rest of the paper, we refer to these discrete representations as ``units''. We extracted representations from the 9$^{th}$ layer of HuBERT model and set $k=200$. Following~\citet{gslm}, repeated units were omitted (e.g., $0,0,0,1,1,2 \rightarrow 0,1,2$). We denote such sequences by ``deduped''. We chose HuBERT for the phonetic-content units as it was shown to better disentangle between speech content and both speaker and prosody compared to other \ac{SSL}-based models~\cite{gslm2}.

\paragraph{Prosodic representation.}
% Duration. 
% A major part of converting emotions is the modeling of prosodic features such as phoneme durations, F0 and voice timbre.
We consider the prosodic representation as a tuple of both content unit durations and F0. 

We start by describing the duration prediction process.
Due to working on deduped sequences, to synthesize the time-domain signal, we first need to predict the duration of each phonetic-content unit.
We follow a similar approach to the one proposed in~\cite{fastspeech2} and use a \ac{CNN} to learn the mapping between content units to durations. We denote this model by $E_{dur}$.
During training, we input the deduped content units $\zc$ and use the ground-truth content unit durations $\zdur$ as supervision. We minimize the \ac{MSE} between the network's output and the target durations. 
% Formally, we minimize,
% \begin{align}
%     L_{dur}(\zc, \zdur) = MSE(E_{dur}(\zc), \zdur).
% \end{align}
We also evaluated n-gram-based duration prediction models. The n-gram models were trained by counting the mean frequency $\mu$ and the standard deviation $\sigma$ of each n-gram in the training set. During inference, we predict the duration of each n-gram by sampling from $\mathcal{N}(\mu, \sigma)$. For unseen n-grams we back-off to a smaller n-gram model. We train a duration model for each target emotion.

\begin{figure}[t!]
\centering
\resizebox{0.49\textwidth}{!}{%
%   \includegraphics[width=\linewidth]{figs/model_overview.png} 
  \includegraphics[width=\linewidth]{figs/model_zoom.png}  
}
\caption{An illustration of the sequence-to-sequence emotion translation component $E_{s2s}$. Here different encoders and decoders are used for each emotions, but we also tested shared architectures in Appendix \ref{sup:add_res}. }
\vspace{-0.3cm}
\label{fig:arch_s2s}
\end{figure}


% \paragraph{F0 Encoder} model is applied over the F0 extracted from the input signal to generate a discrete F0 representation, $\vz_{F0}=(z_{F0}^1, \dots, z_{F0}^{T'})$. Each element in $\vz_{F0}$ is an integer $z_{F0}^i\in\{1,\dots,K'\}$, where $K'$ is the F0 encoder dictionary size. There are various ways to extract the F0 from the input signal, to name a few, YAAPT~\cite{yaapt}, RAPT~\cite{talkin1995robust}, and CREPE~\cite{kim2018crepe}. Similarly, $E_{F_0}$ can be modeled using various ways such as uniform quantization, adaptive quantization, or even a VQ-VAE~\cite{van2017neural, gslm2} model. In this work, we use YAAPT and evaluate several quantization methods (see Table~\ref{tab:f0}). 

We now turn to describe the F0 prediction process.
The relation between emotion, emotion perception and the fundamental frequency (F0) was extensively studied in the psychoacoustics literature \cite{probst2019effects,busso2009fundamental,mcroberts1995role}. Thus, modeling F0 is a crucial step for generating expressive natural speech. To that end, we use a F0 estimation model to predict the pitch from a sequence of discrete units $\zc$. Notice, the mapping between discrete unit sequences and F0 curves is one-to-many, as it depends on the target emotion. Hence, we additionally condition the F0 model on the target emotion denoted by $\zemo^{tgt}$.

Our model, denoted by $E_{F0}$, is a \ac{CNN}, followed by a linear layer projecting the output to $\mathbb{R}^{d}$. The final activation layer is set to be a sigmoid such that the network outputs a vector in $[0,1]^{d}$. 
We extract the ground-truth F0 values from the waveform using the YAAPT~\cite{yaapt} algorithm. Next, we normalize the F0 values using the mean and standard deviation per speaker. We follow a similar approach to~\citet{kim2018crepe} and discretize the range of F0 values into $d$ bins represented by one-hot encodings. Next, we apply Gaussian-blur on these encodings to get the final targets denoted by $\vz_{F0}=(z_{F0}^1, \dots, z_{F0}^{T'})$ where each $z_{F0}^i \in [0,1]^d$. In all experiments, we set $d=50$. Formally, we minimize the binary-cross-entropy (BCE) for each coordinate of the target and the network output,
\vspace{-0.3cm}
\begin{align}
    L_{F0} = \sum_{i=1}^{d} BCE(E_{F0}(\zc, \zemo^{tgt})_i, \vz_{F0}^i).
\end{align}
During inference multiple frequency bins can be activated to a different extent, similarly to \citet{kim2018crepe} we output the F0 value corresponding to the weighted-average of the activated bins. This modeling allows for a better output range when converting bins back to F0 values, as opposed to a single representative F0 value per bin. For F0-to-bin conversion, we use an adaptive binning strategy such that the probability mass of each bin is the same, similarly to~\citet{gslm3}. For completeness, we explored uniform binning, results are summarized in Table~\ref{tab:f0}. Additional log-F0 estimation results are presented in Table~\ref{tab:f0_log} Appendix \ref{sup:add_res}.

% \paragraph{F0 Encoder} model is applied over the F0 extracted from the input signal to generate a discrete F0 representation, $\vz_{F0}=(z_{F0}^1, \dots, z_{F0}^{T'})$. Each element in $\vz_{F0}$ is an integer $z_{F0}^i\in\{1,\dots,K'\}$, where $K'$ is the F0 encoder dictionary size. There are various ways to extract the F0 from the input signal, to name a few, YAAPT~\cite{yaapt}, RAPT~\cite{talkin1995robust}, and CREPE~\cite{kim2018crepe}. Similarly, $E_{F_0}$ can be modeled using various ways such as uniform quantization, adaptive quantization, or even a VQ-VAE~\cite{van2017neural, gslm2} model. In this work, we use YAAPT and evaluate several quantization methods (see Table~\ref{tab:f0}). 

\paragraph{Speaker representation.}
Our goal is to convert the speech emotion while keeping the speaker identity fixed. To that end, we construct a speaker-representation $\zspk$, and include it as an additional conditioner during the waveform synthesis phase. To learn $\zspk$ we optimize the parameters of a fixed size look-up-table. Although such modeling limits our ability to generalize to new and unseen speakers, it produces higher quality generations~\cite{gslm2}. 
We additionally experimented with representing $\zspk$ as a \emph{d-vector} using a method similar to~\citet{heigold2016end}. However, we observed that such approach keeps source emotion prosodic features, resulting in inferior disentanglement during the waveform synthesis phase.


\subsection{Speech Emotion Conversion}
\label{sec:speech_modeling}
We propose to synthesize the speech signal in the target emotion, using the decomposed representation described in the previous paragraph.

We use a translation model to convert between phonetic-content units of a source emotion to phonetic-content units of the target emotion. This serves as a learnable insertion/deletion/substitution mechanism for non-verbal vocalizations, while preserving the lexical content (e.g., removing yawning while preserving the verbal content). Next, we predict the prosodic features (duration and F0) based on the translated units, and inflate the sequence according to the predicted durations. This will later be used as a conditioning for the waveform synthesis phase. 

% \paragraph{Unit Translation.}
To translate the speech content units, we use a sequence-to-sequence Transformer model~\cite{trans} denoted by $E_{s2s}$. The input to $E_{s2s}$ is a sequence of phonetic-content units representing a speech utterance in the source emotion $\zc^{src}$.
The model is trained to output a sequence of phonetic-content units $\zc^{tgt}$ containing the same lexical content with the addition/deletion/substitution of speech cues related to emotion expression (e.g., inserting laughter units).
The optimization minimizes the cross-entropy (CE) loss between the predicted units and ground-truth units for each location in the sequence,
\begin{align}
\label{eq:s2s}
    L_{s2s} = \sum_{i=1}^{L} CE(E_{s2s}( {\zc^{src}, \zemo)}_i, {\zc^{tgt}}_i).
\end{align}
In our experiments, we observed that directly optimizing the above model for translation captures emotion transfer, but fails to maintain the same lexical content, producing expressive yet unintelligible speech utterances (e.g., the model adds laughter but corrupts the sentence by removing needed syllables). To mitigate this, we pre-train the translation model on the task of language denoising auto-encoder similarly to BART \cite{bart}. To better support translation between all emotions we use a dedicated encoder and decoder for each emotion (see Figure~\ref{fig:arch_s2s}). We additionally evaluated a shared-encoder and shared-decoder model, in which we condition on the target emotion, as well as a model where only the encoder is shared. We evaluated all approaches, results are summarized in Table~\ref{tab:arch} Appendix \ref{sup:add_res}.

Next, using the translated phonetic-content unit sequence $\hat{\zc}=E_{s2s}({\zc^{src}, \zemo)}$, we predict the prosodic features corresponding to the target emotion. Formally, 
$\hat{\zdur}=E_{dur}({\hat{\zc}}, \zemo)$ and $\hat{\zf}=E_{F0}(\hat{\zc}, \zemo)$. Recall, as the proposed method is applied over deduped sequences, $\hat{\zc}$ first needs to be inflated according to the predicted durations, for brevity we use the same notation for the inflated $\hat{\zc}$.

Finally, we synthesize the speech signal in the target emotion from $(\hat{\zc}, \hat{\zf}, \zspk, \zemo)$. We follow~\citet{gslm2}, and use a variation of the HiFi-GAN neural vocoder~\cite{kong2020hifi}. The architecture of HiFi-GAN consists of a generator $G$ and a set of discriminators $D$. We adapt the generator component to take as input a sequence of phonetic-content units, F0, the target speaker-embedding, and a target emotion-label, namely $\zc, \zf, \zspk,  \zemo$. The above features are concatenated along the temporal axis and fed into a sequence of convolutional layers that output a 1-dimensional signal. The sample rates of unit sequence and F0 are matched by means of linear interpolation, while the speaker-embedding and emotion-label are replicated.

The discriminators are comprised of two sets: Multi-Scale Discriminators (MSD) and Multi-Period Discriminators (MPD). The first type operates on different sizes of a sliding window over the signal (2, 4), while the latter samples the signal at different rates (2,3,5,7,11). Overall, each discriminator $D_i$ is trained by minimizing the following loss function,
\begin{align}
    & L_{adv}(D_i, G) = \sum_{\x} || 1 - D_i(\xhat) ||^2_2 \\
    & L_D(D_i, G) = \sum_{\x} || 1 - D_i(\x) ||^2_2 + || D_i(\xhat) ||^2_2 \notag
\end{align}
where $\xhat = G(\zc, \zf, \zspk, \zemo)$ is the time-domain signal reconstructed from the disentangled representation. There are two additional loss terms used for optimizing $G$. The first is a Mean-Absolute-Error (MAE) reconstruction loss in the log-mel frequency domain $L_{recon}(G) = \sum_{\x} || \phi(\x) - \phi(\xhat) ||_1$.
% \begin{align}
%     & L_{recon}(G) = \sum_{\x} || \phi(\x) - \phi(\xhat) ||_1
% \end{align}
where $\phi$ is the spectral operator computing the Mel-spectrogram. The second loss term is a feature matching loss, which penalizes for large discrepancies in the intermediate discriminator representations, $L_{fm}(D_i, G) = \sum_{\x}\sum^{R}_{j=1} || \xi_j(\x) - \xi_j(\xhat) ||_1$
% \begin{align}
%     & L_{fm}(D_i, G) = \sum_{\x}\sum^{R}_{j=1} || \xi_j(\x) - \xi_j(\xhat) ||_1
% \end{align}
where $\xi_j$ is the operator that extracts the intermediate representation of the $j$th layer of discriminator $D_i$ with $R$ layers.
The overall objective for optimizing the system is:
\vspace{-0.2cm}
\begin{align}
    L_G(D,G) &= \bigg[ \sum_{i=1}^J L_{adv}(D_i, G) + \lambda_{fm} L_{fm}(D_i, G)\bigg] \notag \\ 
    &+ \lambda_{r} L_{recon}(G), \notag \\
    L_D(D,G) &= \sum_{i=1}^J L_D(D_i, G),
\end{align}
where $\lambda_{fm}=2$ and $\lambda_r=45$. 

We observed that adding an emotion-token is crucial for generating expressive speech. This token captures voice timbre expressing emotion characteristics, such as roughness, smoothness, etc.






% \vspace{-0.1cm}
% \section{Model}
% \label{sec:model}
% Emotion can manifest itself in multiple aspects: the prosody may reflect emotion via high pitch or a certain rythem. Additionally  
% We propose to decompose the speech signal into four components: content, prosodic features (i.e., F0 and duration), speaker identity, and emotion-token denoted by $\zc, (\zdur, \zf), \zspk, \zemo$ respectively. Our model is composed of multiple components, each handling a different aspect of the above decomposition.
% To represent the speech content we extract a discrete representation of the audio signal using a pre-trained self-supervised model, namely HuBERT. Consecutive occurrences of the same token are collapsed to a single token.
% Next, we feed this representation to a sequence-to-sequence Transformer model optimized for translating discrete representations of different emotions. We predict the durations of each token in the translated output sequence and inflate them accordingly. Using a F0 estimation model and the translated tokens, we predict the F0 corresponding to the target emotion. Finally, we feed them together with the target speaker-embedding and target emotion-token to a neural vocoder trained to reconstruct the time-domain audio signal. The overall architecture is depicted in Figure~\ref{fig:arch}.

% \vspace{-0.1cm}
% \subsection{Speech-to-Units}
% \noindent{\textbf{Content Encoder.}}
% Denote the domain of audio samples by $\mathcal{X} \subset \mathbb{R}$. The representation for an audio waveform is therefore a sequence of samples $\x = (x^1, \dots, x^T)$, where each $x^i \in \mathcal{X}$ for all $1 \leq t \leq T$. The content encoder $E_c$ is a HuBERT model \cite{hsu2020hubert} pre-trained on the LibriSpeech corpus~\cite{Panayotov2015}. HuBERT is a self-supervised model trained on the task of masked prediction of continuous audio signals, similarly to BERT~\cite{bert}. During training, the targets are obtained via clustering of MFCCs features or learned representations from earlier iterations.
% The input to the content encoder $E_c$ is an audio waveform $\x$, and the output is a spectral representation sampled at a lower frequency $\z' = (z_c^{'1}, \dots, z_c^{'L})$ where $L < T$. Since HuBERT outputs continuous representations, an additional k-means step is needed in order to quantize these representations into a discrete token sequence denoted by $\zc = (z_c^1, \dots, z_c^L)$ where $z_c^i \in \{1, \dots, K\}$ and $K$ is the size of the vocabulary. In this study, we extracted representations from the 9$^{th}$ layer of HuBERT model and set $k=200$.


% \paragraph{F0 Encoder} model is applied over the F0 extracted from the input signal to generate a discrete F0 representation, $\vz_{F0}=(z_{F0}^1, \dots, z_{F0}^{T'})$. Each element in $\vz_{F0}$ is an integer $z_{F0}^i\in\{1,\dots,K'\}$, where $K'$ is the F0 encoder dictionary size. There are various ways to extract the F0 from the input signal, to name a few, YAAPT~\cite{yaapt}, RAPT~\cite{talkin1995robust}, and CREPE~\cite{kim2018crepe}. Similarly, $E_{F_0}$ can be modeled using various ways such as uniform quantization, adaptive quantization, or even a VQ-VAE~\cite{van2017neural, gslm2} model. In this work, we use YAAPT and evaluate several quantization methods (see Table~\ref{tab:f0}). 

% \paragraph{Speaker Encoder.}
% Our goal is to convert the speech emotion while keeping the speaker identity fixed. To that end, we construct a speaker-representation $\zspk$, and include it as an additional conditioner during the waveform synthesis phase. To learn $\zspk$ we optimize the parameters of a fixed size look-up-table. Although such modeling limits our ability to generalize to new and unseen speakers, it produces higher quality generations~\cite{gslm2}. 

% We additionally experimented with representing $\zspk$ as a \emph{d-vector} using a method similar to~\citet{heigold2016end}. However, we observed that such approach keeps source emotion prosodic features, resulting in inferior disentanglement during the waveform synthesis phase.


% \subsection{Speech Modeling}
% \label{sec:speech_modeling}
% In this work, we propose to \emph{regenerate} speech in a target emotion, using the decomposed representation described in the previous paragraph.
% We use a translation model to convert between speech units of a source emotion to speech units of the target emotions. This serves as a learnable insertion/deletion/substitution mechanism for non-verbal vocalizations. Next, we predict the prosodic features (duration and F0) based on the translated units, and inflate the sequence according to the predicted durations. This will later be used as a conditioning for the waveform synthesis phase. 

% \paragraph{Unit Translation.}
% To translate the speech content units, we use a sequence-to-sequence Transformer model~\cite{trans} denoted by $E_{s2s}$. The input to $E_{s2s}$ is a sequence of units representing a speech utterance in the source emotion $\zc^{src}$.
% The model is trained to output a sequence of units $\zc^{tgt}$ containing the same lexical content with the addition/deletion/substitution of speech cues related to emotion expression (e.g., inserting laughter units).
% The optimization minimizes the cross-entropy (CE) loss between the predicted units and ground-truth units for each location in the sequence,
% \begin{align}
% \label{eq:s2s}
%     L_{s2s} = \sum_{i=1}^{L} CE(E_{s2s}( {\zc^{src})}_i, {\zc^{tgt}}_i).
% \end{align}
% In our experiments, we observed that directly optimizing the above model for translation captures emotion transfer, but fails to maintain the same lexical content, producing expressive yet unintelligible speech utterances. To mitigate this, we pre-train the translation model on the task of language denoising (a form of auto-encoding) similarly to BART \cite{bart}. Following~\citet{gslm}, during both pre-training and fine-tuning the model operates on sequences where repeating units were omitted (e.g., $0,0,0,1,1,2 \rightarrow 0,1,2$). We denote such sequences by ``deduped''. To better support translation between all emotions we setup a dedicated encoder and decoder for each emotion (see Figure~\ref{fig:arch_s2s}). We also evaluated a shared-encoder and shared-decoder model, in which we condition on the target emotion, as well as a model where only the encoder is shared. We evaluated all approaches, results are summarized in Table~\ref{tab:arch} Appendix \ref{sup:add_res}. 
% %  as well as a shared encoder only architecture.

% % We evaluated three weight-sharing schemes for this model: (i) all emotions use the same encoder and decoder components of the Transformer architecture. In this case, we condition the model on the target emotion. This can be done by prepending a special target emotion token at the beginning of the decoding procedure. We denote this approach by ``share-all''. (ii) All emotions share the same encoder but have separate dedicated decoders. In this case, no target emotion conditioning is needed. We denote this approach by ``share-enc''. Finally, (iii) each emotion has a dedicated encoder and decoder. We denote this approach by ``share-none''. We evaluated all three approaches and summarized the results in Table~\ref{tab:arch} on Appendix \ref{sup:add_res}. 


% \paragraph{Duration Predictor}.
% A major part of converting emotions is the modeling of prosodic features such as phoneme durations, F0 and voice timbre.
% Due to working on deduped sequences, to reconstruct the time-domain signal, we first need to predict the duration of each speech unit.
% We follow a similar approach to the one proposed in~\cite{fastspeech2} and use a \ac{CNN} to learn the mapping between input units to durations. We denote this model by $E_{dur}$.
% During training, we input the deduped units $\zc$ and use the ground-truth unit durations $\zdur$ as supervision. We minimize the \ac{MSE} between the network's output and the target durations. 
% % Formally, we minimize,
% % \begin{align}
% %     L_{dur}(\zc, \zdur) = MSE(E_{dur}(\zc), \zdur).
% % \end{align}
% We also evaluated n-gram-based duration prediction models. The n-gram models were trained by counting the mean frequency $\mu$ and the standard deviation $\sigma$ of each n-gram in the training set. During inference, we predict the duration of each n-gram by sampling from $\mathcal{N}(\mu, \sigma)$. For unseen n-grams we back-off to a smaller n-gram model.

% \begin{figure}[t!]
% \centering
% \resizebox{0.49\textwidth}{!}{%
% %   \includegraphics[width=\linewidth]{figs/model_overview.png} 
%   \includegraphics[width=\linewidth]{figs/model_zoom.png}  
% }
% \caption{An illustration of the sequence-to-sequence emotion translation component $E_{s2s}$. Here different encoders and decoders are used for each emotions, but we also tested shared architectures in Appendix \ref{sup:add_res}. }
% \vspace{-0.3cm}
% \label{fig:arch_s2s}
% \end{figure}

% \paragraph{F0 Predictor}.
% The relation between emotion, emotion perception and the fundamental frequency (F0) was extensively studied in the psychoacoustics literature \cite{probst2019effects,busso2009fundamental,mcroberts1995role}. Thus, modeling F0 is a crucial step for generating expressive natural speech. To that end, we use a F0 estimation model to predict the pitch from a sequence of discrete units $\zc$. Notice, the mapping between discrete unit sequences and F0 curves is one-to-many, as it depends on the target emotion. Hence, we additionally condition the F0 model on the target emotion denoted by $\zemo^{tgt}$.

% Our model is a \ac{CNN}, followed by a linear layer projecting the output to $\mathbb{R}^{d}$. The final activation layer is set to be a sigmoid such that the network outputs a vector in $[0,1]^{d}$. 
% We extract the ground-truth F0 values from the waveform using the YAAPT algorithm. Next, we normalize the F0 values using the mean and standard deviation per speaker. We follow a similar approach to~\citet{kim2018crepe} and discretize the range of F0 values into $d$ bins represented by one-hot encodings. Next, we apply Gaussian-blur on these encodings to get the final targets denoted by $\vz_{F0}=(z_{F0}^1, \dots, z_{F0}^{T'})$ where each $z_{F0}^i \in [0,1]^d$. In all experiments, we set $d=50$. Formally, we minimize the binary-cross-entropy (BCE) for each coordinate of the target and the network output,
% \vspace{-0.3cm}
% \begin{align}
%     L_{F0} = \sum_{i=1}^{d} BCE(E_{F0}(\zc, \zemo^{tgt})_i, \vz_{F0}^i).
% \end{align}
% During inference multiple frequency bins can be activated to a different extent, similarly to \citet{kim2018crepe} we output the F0 value corresponding to the weighted-average of the activated bins. This modeling allows for a better output range when converting bins back to F0 values, as opposed to a single representative F0 value per bin. For F0-to-bin conversion, we use an adaptive binning strategy such that the probability mass of each bin is the same, similarly to~\citet{gslm3}. For completeness, we explored uniform binning, results are summarized in Table~\ref{tab:f0}. Additional log-F0 estimation results are presented in Table~\ref{tab:f0_log} Appendix \ref{sup:add_res}.


% \paragraph{Units-to-Speech}.
% Similarly to~\citet{gslm2}, we use a variation of the HiFi-GAN neural vocoder~\cite{kong2020hifi}. The architecture of HiFi-GAN consists of a generator $G$ and a set of discriminators $D$. We adapt the generator component to take as input a sequence of discrete units, F0, the target speaker-embedding, and a target emotion-token, namely $\zc, \zf, \zspk,  \zemo$. The above features are concatenated along the temporal axis and fed into a sequence of convolutional layers that output a 1-dimensional signal. The sample rates of unit sequence and F0 are matched by means of linear interpolation, while the speaker-embedding and emotion-token are replicated.

% The discriminators are comprised of two sets: Multi-Scale Discriminators (MSD) and Multi-Period Discriminators (MPD). The first type operates on different sizes of a sliding window over the signal (2, 4), while the latter samples the signal at different rates (2,3,5,7,11). Overall, each discriminator $D_i$ is trained by minimizing the following loss function,
% \begin{align}
%     & L_{adv}(D_i, G) = \sum_{\x} || 1 - D_i(\xhat) ||^2_2 \\
%     & L_D(D_i, G) = \sum_{\x} || 1 - D_i(\x) ||^2_2 + || D_i(\xhat) ||^2_2 \notag
% \end{align}
% where $\xhat = G(\zc, \zf, \zspk, \zemo)$ is the time-domain signal reconstructed from the disentangled representation. There are two additional loss terms used for optimizing $G$. The first is a Mean-Absolute-Error (MAE) reconstruction loss in the log-mel frequency domain $L_{recon}(G) = \sum_{\x} || \phi(\x) - \phi(\xhat) ||_1$.
% % \begin{align}
% %     & L_{recon}(G) = \sum_{\x} || \phi(\x) - \phi(\xhat) ||_1
% % \end{align}
% where $\phi$ is the spectral operator computing the Mel-spectrogram. The second loss term is a feature matching loss, which penalizes for large discrepancies in the intermediate discriminator representations, $L_{fm}(D_i, G) = \sum_{\x}\sum^{R}_{j=1} || \xi_j(\x) - \xi_j(\xhat) ||_1$
% % \begin{align}
% %     & L_{fm}(D_i, G) = \sum_{\x}\sum^{R}_{j=1} || \xi_j(\x) - \xi_j(\xhat) ||_1
% % \end{align}
% where $\xi_j$ is the operator that extracts the intermediate representation of the $j$th layer of discriminator $D_i$ with $R$ layers.
% The overall objective for optimizing the system is:
% \vspace{-0.2cm}
% \begin{align}
%     L_G(D,G) &= \bigg[ \sum_{i=1}^J L_{adv}(D_i, G) + \lambda_{fm} L_{fm}(D_i, G)\bigg] \notag \\ 
%     &+ \lambda_{r} L_{recon}(G), \notag \\
%     L_D(D,G) &= \sum_{i=1}^J L_D(D_i, G),
% \end{align}
% where $\lambda_{fm}=2$ and $\lambda_r=45$. 

% We observed that adding an emotion-token is crucial for generating expressive speech. This token captures voice timbre expressing emotion characteristics, such as roughness, smoothness, etc.

==> results.bak.tex <==
\vspace{-0.5cm}
\section{Results}
\label{sec:results}
\vspace{-0.1cm}
We evaluate the performance of the different components of our system.
We start with the subjective evaluation for the overall system in terms of audio-quality (\ac{MOS}) and the perceived emotions (\ac{eMOC}).
% Next, we evaluate of the translation model using BLEU, \ac{UER}, \ac{WER}, and \ac{PER}.
Next, we evaluate the duration and F0 estimation modules. Finally, we provide an ablation study where we measure the impact of each component on the perceived emotion, and evaluate the configuration for discrete unit extraction. 

Figure~\ref{fig:mos} depicts the \ac{MOS}, and \ac{eMOC} scores for the proposed method and the baselines. Results suggest that the proposed method surpasses the evaluated baselines in terms of MOS and eMOC. 
While Tacotron2 and Seq2seq-EVC succeed in conveying the target emotion, they produce less natural expressive speech utterances, which is reflected in lower MOS. 
Recall, unlike our method, both Tacotron2 and Seq2seq-EVC are text-based systems hence they attempt to learn an alignment (an attention map) between text inputs and audio targets. This task is particularly challenging as non-verbal cues (e.g., laughter, breathing) are not annotated in the text inputs. We hypothesize that this misalignment leads to less natural expressive speech production.

An evaluation of different model design architectures together with \ac{eMOC} confusion matrices for the proposed method, evaluated baselines, and ground truth recordings can be found on the Appendix~\ref{sup:add_res}.

\vspace{-0.1cm}
\subsection{Prosodic Modeling Analysis}
\vspace{-0.1cm}

\begin{table}[t!]
    \centering
    \resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c}
        \toprule
        Quantization & Norm.  & Prediction & MAE \\
        \toprule
         uniform     & \ding{55} & argmax & 83.51 \\ \hline
         uniform     & \ding{55} & w-avg  & 44.92 \\ \hline
         uniform     & mean      & argmax & 53.74 \\ \hline
         uniform     & mean      & w-avg  & 35.63 \\ \hline
         uniform     & mean-std  & argmax & 63.01 \\ \hline
         uniform     & mean-std  & w-avg  & 35.69 \\ \hline
         adaptive    & \ding{55} & argmax & 129.7 \\ \hline
         adaptive    & \ding{55} & w-avg  & 45.21 \\ \hline
         adaptive    & mean      & argmax & 127.8 \\ \hline
         adaptive    & mean      & w-avg  & 36.06 \\ \hline
         adaptive    & mean-std  & argmax & 155.7 \\ \hline
         adaptive    & mean-std  & w-avg  & \bf 35.38 \\
         \bottomrule
    \end{tabular}
    }
    \caption{Evaluation of different F0 estimation configurations. The MAE is reported for voiced frames only.}
    \vskip -1em
    \label{tab:f0}
\end{table}

We now turn to evaluate the F0 estimation model using the \ac{MAE} between ground-truth F0 and predicted F0. In this experiment, we explored a number of configurations for training such an estimator. Specifically, we evaluated different binning strategies, normalization methods and prediction rules. For binning strategies, we explored adaptive binning vs. uniform binning. Under normalization, we explored no normalization, mean normalization and mean \& standard deviation normalization\footnote{The mean and standard deviation are computed using the F0 values per speaker.}. Finally, in addition to the weighted-average prediction rule described in Section~\ref{sec:speech_modeling}, we also evaluate an argmax prediction rule where the highest scoring bin is predicted. Results are summarized in Table~\ref{tab:f0}. 
Results suggest that the weighted-average prediction rule is preferable to argmax, especially when used in conjunction with adaptive binning. This can be explained by large-range bins in the adaptive case, leading to larger \ac{MAE} when selecting a single bin using the argmax operator. Although adaptive quantization reaches the best performance, under specific settings uniform quantization can reach comparable results. For normalization, it is preferable to normalize, the specific normalization method has little impact on performance. 

Next, we evaluate the duration prediction models using the \ac{MAE} between target and predicted durations. For a more complete analysis, we also report the accuracy using thresholds of 0ms, 20ms and 40ms. We explored a \ac{CNN} duration predictor similarly to \cite{fastspeech2} and three n-gram based models. The results are summarized in Table~\ref{tab:dur}.
\begin{table}[t!]
    \centering
    \resizebox{0.95\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c}
        \toprule
        Model & \ac{MAE} & Acc@0ms  & Acc@20ms & Acc@40ms \\
        \toprule
         \ac{CNN}  & \bf 0.77 & \bf 51.12 & \bf 86.24 & \bf 94.08 \\ \hline
         1-gram    & 1.47 & 29.41 & 67.34 & 83.26 \\ \hline
         3-gram    & 1.16 & 36.78 & 76.04 & 88.32 \\ \hline
         5-gram    & 1.02 & 37.32 & 81.36 & 90.46 \\
         \bottomrule
    \end{tabular}}
    \caption{Evaluation of four duration prediction models. CNN architecture is as described in~\cite{fastspeech2}.}
    \vspace{-0.2cm}
    \label{tab:dur}
\end{table}
As expected, the \ac{CNN} outperforms n-gram models, with $\sim$94\% accuracy when considering a tolerance level of 40ms.


\vspace{-0.2cm}
\subsection{Ablation}
\paragraph{Model configuration.}
\citeauthor{yang2021superb} found that intermediate HuBERT representations obtained from different layers have an impact on the downstream task at hand. Specifically, when considering spoken language modeling, \citeauthor{gslm} used the 6$^{th}$ layer, while \citeauthor{gslm3} used layer 9. Additionally, \citeauthor{gslm} showed that the number of units ($k$) also has an impact on the overall performance of the system. 

To better understand the effect of these architectural configurations in our setting, we experimented with extracting HuBERT features from layers 6 and 9, using 100 and 200 clusters for the k-means post-processing step. Additionally, we measure the impact that pre-training the translation model has on performance. As we compare models with different vocabulary sizes, we cannot use metrics such as BLEU and \ac{UER}, hence, we report \ac{WER} and \ac{PER}. Results are in Table~\ref{tab:abl}. 
 
For emotion conversion, we found that using the 9$^{th}$ HuBERT layer and 200 tokens performs best. It can be seen that without pre-training all models fail to generate intelligible speech. This is due to limited number of parallel emotion training pairs. 

\begin{table}[t!]
    \centering
    \resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{c|c|c|c|c}
        \toprule
        \# units & layer no. & pre-trained  & \ac{WER} & \ac{PER} \\
        \toprule
         100    & 6 & \ding{55} & 88.85 & 72.17 \\ \hline
         100    & 6 & \ding{51} & 36.01 & 29.67 \\ \hline
         100    & 9 & \ding{55} & 83.72 & 66.63 \\ \hline
         100    & 9 & \ding{51} & 31.69 & 27.90 \\ \hline
         200    & 6 & \ding{55} & 91.06 & 77.14 \\ \hline
         200    & 6 & \ding{51} & 31.97 & 27.49 \\ \hline
         200    & 9 & \ding{55} & 84.92 & 71.45 \\ \hline
         200    & 9 & \ding{51} & \bf 23.92 & \bf 25.95 \\
         \bottomrule
    \end{tabular}}
    \caption{Evaluation of different token extraction configurations and the effect of pre-training the translation model. \# units denotes the vocabulary size, layer no. denotes the layer index used in HuBERT.}
    \vskip -1em
    \label{tab:abl}
\end{table}

\noindent{\textbf{Different components.}}
Recall, we decompose speech into four disentangled features. The contribution of each feature on the perceived emotion is still left unclear. In this paragraph, we gauge the effect of each feature by gradually adding different components and evaluating their impact on the \ac{eMOC} metric. Specifically, we start by evaluating the source features and replacing the emotion-token. Then, we predict the unit durations and F0 for the target emotion. Lastly, the full effect of our method is achieved by incorporating the unit translation model. For reference, we report results for the original recording, and resynthesized one (i.e., using source features only) and the target recording. Results are summarized in Table~\ref{tab:abl_comp}. 

Results suggest that the proposed method is comparable to ground-truth recordings in terms of the perceived emotion. Interestingly, for the Sleepy emotion, modifying the timbre using the target emotion-token and adjusting the unit durations is enough to reach $70.31\%$, while the rest of the emotions require further processing. For Amused, Angry and Disgusted modifying the F0 reaches performance of $5\%$ below the ground-truth recordings. When applying the entire pipeline results are on par with the ground-truth. This can be explained by the addition and deletion of non-verbal vocalizations by the translation model.

\vspace{-0.1cm}
\subsection{Out-of-distribution samples}
\vspace{-0.1cm}
Due to the size of the EmoV dataset (7000 samples overall) the number of unique utterance is small. As a result, the model can memorize the utterances and might fail to generalize to unseen sentences. Hence, we experimented with converting out-of-domain recordings. To that end, we input our system with recordings from the LibriSpeech dataset. As LibriSpeech consists of non-expressive samples, we treat them as ``neutral''. We convert these samples to different emotions and evaluate the performance. For evaluation we randomly sampled 20 utterances converted to each emotion. The proposed method reaches an average \ac{eMOC} score of $82.25\% \pm7.32$ and an average \ac{MOS} score of $3.69 \pm0.26$ across all four emotions (amused, angry, disgusted, sleepy). When considering the lexical content, the \ac{WER} between the ground-truth text and \ac{ASR} based transcriptions of the generated audio is 27.92. These results are similar to the ones reported for the EmoV dataset.

\begin{table}[t!]
    \centering
    \resizebox{1.0\columnwidth}{!}{%
        \begin{tabular}{c|c|c|c|c|c|c|c}
        \toprule
         \multirow{2}{*}{Tokens} & \multirow{2}{*}{Emotion} & \multirow{2}{*}{F0} & \multirow{2}{*}{Duration} & \multicolumn{4}{c}{\ac{eMOC}} \\
         & & & & Amused & Angry & Disgusted & Sleepy\\
        \toprule
        \multicolumn{4}{c|}{Original -- Neutral}        & 20.11 & 21.66 & 7.59 & 17.34  \\ \midrule \midrule
        src  & src   & src  & src                       & 20.24 & 18.62 & 8.37 & 17.72   \\ \midrule
        src  & tgt   & src  & src                       & 27.66 & 25.76 & 10.83 & 25.19  \\ \midrule
        src  & tgt   & src  & pred                       & 30.89 & 35.71 & 32.11 & 70.31 \\ \midrule
        src  & tgt   & pred & pred                      & 79.12 & 86.11 & 69.21 & 79.12  \\ \midrule
        pred & tgt   & pred & pred                      & 85.16 & 90.61 & 75.89 & 84.23  \\ \midrule\midrule
        \multicolumn{4}{c|}{Original -- Emotion}        & 86.31 & 89.92 & 76.18 & 88.01  \\ 
         \bottomrule
    \end{tabular}}
    \caption{Effect of components in our system on perceived emotion. ``Original -- Neutral'' denotes the ground-truth neutral recordings while ``Original -- Emotion'' denotes the ground-truth emotional recording. ``src'', ``tgt'', and ``pred'' denote features extracted from source speech, features extracted from target speech, and features predicted by our system respectively.}
    \vskip -1em
    \label{tab:abl_comp}
\end{table}

==> stuff2bring.back.tex <==
% The relation between emotion, emotion perception and the fundamental frequency (F0) was extensively studied in the psychoacoustics literature \cite{probst2019effects,busso2009fundamental,mcroberts1995role}. Thus, modeling F0 is a crucial step for generating expressive natural speech. 
